Adversarially Robust Medical Classification via Attentive Convolutional Neural Networks

Convolutional neural network-based medical image classifiers have been shown to be especially susceptible to adversarial examples. Such instabilities are likely to be unacceptable in the future of automated diagnoses. Though statistical adversarial example detection methods have proven to be effective defense mechanisms, additional research is necessary that investigates the fundamental vulnerabilities of deep-learning-based systems and how best to build models that jointly maximize traditional and robust accuracy. This paper presents the inclusion of attention mechanisms in CNN-based medical image classifiers as a reliable and effective strategy for increasing robust accuracy without sacrifice. This method is able to increase robust accuracy by up to 16% in typical adversarial scenarios and up to 2700% in extreme cases.

==> figures/XRayProcessingPipeline.tex <==
\begin{figure}[h]
    \centering
    $
    \begin{array}{l}
    \includegraphics[width=0.4\linewidth]{graphics/ResNet-50/unprocessedxray.png}
    \end{array}
    \mathlarger{\mathlarger{\mathlarger{\mathlarger{\rightarrow}}}}
    \begin{array}{l}
        \includegraphics[width=0.4\linewidth]{graphics/ResNet-50/processedxray.jpg}
    \end{array}
    $
    \caption{Visualization of the chest x-ray image preprocessing pipeline}
\end{figure}

==> paper for arxiv/figures/DRPerturbationDivergence.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}{.4\linewidth}
      \centering
      \includegraphics[width=\linewidth]{graphics/ResNet-50/LesionOutline.pdf}
      \caption{Shape of skin lesion found in adversarial ``noise''\\}
      \label{LesionShape}
    \end{subfigure}
    \begin{subfigure}{.4\linewidth}
      \centering
      \includegraphics[width=\linewidth]{graphics/ResNet-50/EyeShapeDivergence.pdf}
      \caption{Divergence from shape of eye\\}
      \label{EyeShapeDivergence}
    \end{subfigure}
    \caption{Shape information carried over into perturbations}
  \end{figure}

==> paper for arxiv/figures/ResNetCottonWool.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{graphics/ResNet-50/cotton_wool.pdf}
    \caption{Dark splotches in perturbation of fundoscopic images}
    \label{CottonWool}
  \end{figure}

==> paper for arxiv/figures/ResNetPneumoWithAttentionActivation.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{graphics/ResNet-50/pneumo_with_attention.pdf}
    \caption{Comparison of activation maps (with attention) for perturbed and unperturbed chest x-ray}
    \label{PneumoWithAttention}
  \end{figure}

==> paper for arxiv/figures/ResNetPneumoWithoutAttentionActivation.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{graphics/ResNet-50/different_maps.pdf}
    \caption{Comparison of activation maps (without attention) for perturbed and unperturbed chest x-ray}
    \label{DifferentMaps}
  \end{figure}

==> paper for arxiv/figures/XRayProcessingPipeline.tex <==
\begin{figure}[h]
    \centering
    $
    \begin{array}{l}
    \includegraphics[width=0.4\linewidth]{graphics/ResNet-50/unprocessedxray.png}
    \end{array}
    \mathlarger{\mathlarger{\mathlarger{\mathlarger{\rightarrow}}}}
    \begin{array}{l}
        \includegraphics[width=0.4\linewidth]{graphics/ResNet-50/processedxray.jpg}
    \end{array}
    $
    \caption{Visualization of the chest x-ray image preprocessing pipeline}
\end{figure}
